A novel approach to model exploration for value function learning

Planning and Learning are complementary approaches. Planning relies on deliberative reasoning about the current state and sequence of future reachable states to solve the problem. Learning, on the other hand, is focused on improving system performance based on experience or available data. Learning to improve the performance of planning based on experience in similar, previously solved problems, is ongoing research. One approach is to learn Value function (cost-to-go) which can be used as heuristics for speeding up search-based planning. Existing approaches in this direction use the results of the previous search for learning the heuristics. In this work, we present a search-inspired approach of systematic model exploration for the learning of the value function which does not stop when a plan is available but rather prolongs search such that not only resulting optimal path is used but also extended region around the optimal path. This, in turn, improves both the efficiency and robustness of successive planning. Additionally, the effect of losing admissibility by using ML heuristic is managed by bounding ML with other admissible heuristics.

==> macros/packages.tex <==
%============================================================================
% The following packages can be found on http:\\www.ctan.org
% BIBTEX
%\usepackage{cite}
% BIBLATEX: \usepackage[style=IEEEtran,backend=bibtex]{biblatex}

\usepackage{graphicx}  % for pdf, bitmapped graphics files
\usepackage{array}
%\usepackage{epsfig}   % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times}     % assumes new font selection scheme installed
\usepackage[fleqn]{amsmath}   % assumes amsmath package installed
\usepackage{amssymb}   % assumes amsmath package installed
%\usepackage{mathabx}   % for \widebar % Böse (font 3)
\usepackage{dsfont}
\usepackage{float}     % for placing with (H) at a specific position 
\usepackage{textgreek}
\usepackage[table]{xcolor}  % Färbige Tabellen
\usepackage{booktabs}       % Schöne Tabellen (dicke und dünne Linien)
\usepackage{filemod}        % für autoupdate bei geänderten tikz-grafiken
\usepackage{xifthen}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{footnote}
%==============================================================================
% macro for executing a shell command immidiatly 
%\newcommand{\runmycommand}[1]{\immediate\write18{#1}}
% AUTOMATIC BIBTEX
\IfFileExists{\jobname.aux}% needs --enable-write18
             {\typeout{bibtex \jobname.aux}
              \immediate\write18{bibtex \jobname.aux}
              \typeout{*** AUTO RUNNING BIBTEX ***}}
             {\typeout{*********** Rerun for bibliography *************}}
%FOR BIBLATEX %\addbibresource{./IEEEabrv,./library}
             
% Pakete für Blockdiagramme und Diagramme
\usepackage{tikz}               % Achtung die Reihenfolge der Tikz Pakete ist
\usepackage{pgfplots}           % entscheidend!
\usepackage{pgfplotstable} 
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{units}
%\usetikzlibrary{spy}
\usetikzlibrary{shadows,positioning,arrows}
%\usetikzlibrary{shapes,shapes.multipart}
\usetikzlibrary{calc}
\usetikzlibrary{trees,fit,backgrounds}
%\usetikzlibrary{patterns,decorations.pathreplacing,decorations.pathmorphing}
%\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur,shapes.symbols}

%=================================================================================
\usepgfplotslibrary{external} % PDFs machen
\tikzexternalize[prefix=tikz_temp/]     % Unterordner für PDFs
\newcommand\autoupdateexternfigure[2]{  % MAKRO UM AUTOUPDATE ZU ERMÖGLICHEN
  \tikzsetnextfilename{#2}              % pdf-filename
  \filemodCmp{#1}{tikz_temp/#2.log}%    % prüft file datum 
  {\tikzset{external/force remake=true}}% erzwingt remake wenn log alt
  {}
}
%\tikzset{external/force remake} % immer alle Bilder neu machen
% Achtung für später: EPS-Grafiken können mit Tikz auch automatisch erstellt werden (siehe Internet)
% Tipps zu eps: auf http://tex.stackexchange.com/questions/8641/export-eps-figures-from-tikz
%=================================================================================

% Spezial Worttrennungen
\hyphenation{Last-rampen Betriebs-punkt}

%============================================================================
% PDF-Einstellungen
%\usepackage[ pdfauthor={Zlatan Ajanovic, Michael Stolz, Martin Horn}
%             ,pdftitle={A Novel Observer Concept for Embedded Drivetrain Applications}
%             ,pdfpagelayout=TwoPageLeft
%             ,pdfstartview  = {FitV}
%             %,pdfpagemode  = UseAttachments %OPEN ATTACHMENTS-VIEW IN PD
%             ,pdfpagelabels = true
%             ,linkcolor     = {black}
%             ,colorlinks    = {true} 
%             ,citecolor     = {black}
%             ,urlcolor      = {black}
%             ,bookmarks, bookmarksnumbered
%             %,bookmarksopen={true}, 
%             %,pagebackref  = true, backref = page     %% turn on backreferencing
%             ,plainpages    = false
%             ,hypertexnames = true
%             ]{hyperref}
%============================================================================
% Matrizen ------------------------------------------------------------------  
%\usepackage{arydshln}         % have dotted lines to separate matrix elements 
%\newcommand{\myhdots}{\hdashline[.4pt/1.5pt]}          % macro für punktierte

==> macros/symbols3.tex <==
\newcommand{\mymatrix}[1]{\mathbf{#1}}
\newcommand{\myvector}[1]{\mathbf{#1}}
\newcommand{\mytransf}[1]{#1}
\newcommand{\myfarg}[1]{\mbox{\footnotesize$({#1})$}}
\newcommand{\mysub}[1]{_{\!\:\!#1}}

\newcommand{\A}{\mymatrix{A}}
\newcommand{\B}{\mymatrix{B}}
\newcommand{\C}{\mymatrix{C}}
\newcommand{\D}{\mymatrix{D}}
\newcommand{\F}{\mymatrix{F}}
\newcommand{\E}{\mymatrix{E}}
\newcommand{\Mmass}{\mymatrix{M}}

\newcommand{\K}{\mymatrix{K}}
\newcommand{\Id}{\mymatrix{I}}
\newcommand{\G}{\mymatrix{G}}
\newcommand{\SM}{\mymatrix{S}}
\newcommand{\PHI}{\boldsymbol\Phi}
\newcommand{\XI}{\boldsymbol\Lambda}
\newcommand{\HH}{\mymatrix{H}}

\newcommand{\LL}{\mymatrix{L}}
\newcommand{\T}{\tau}
\newcommand{\TT}{\boldsymbol\tau}
\newcommand{\M}{\mymatrix{M}}
\newcommand{\R}{\mytransf{R}}
\newcommand{\PP}{\mymatrix{P}}
\newcommand{\x}{\myvector{x}}
\newcommand{\dd}{\myvector{d}}
\newcommand{\e}{\myvector{e}}
\newcommand{\f}{\myvector{f}}
\newcommand{\uu}{\myvector{u}}
\newcommand{\z}{\myvector{z}}
\newcommand{\rr}{\myvector{r}}  
\newcommand{\y}{\myvector{y}} 
\newcommand{\vv}{\myvector{v}} 
\newcommand{\V}{\mymatrix{V}}
\newcommand{\U}{\mytransf{U}}
\newcommand{\X}{\mymatrix{X}}
\newcommand{\Q}{\mytransf{Q}}
\newcommand{\Z}{\mytransf{Z}}
\newcommand{\w}{\myvector{w}}


\newcommand{\q}{\mathbf{q}}
\newcommand{\mylam}[2]{\lambda_{(\mathit{#1},#2)}}
\newcommand{\mytau}[2]{\tau_{(\mathit{#1},#2)}}

\newcommand{\Teng}{\T_{\!\mathit{eng}}}
\newcommand{\Tmot}{\T_{\!\mathit{eng}}}
\newcommand{\Tveh}{\T_{\!\mathit{veh}}}
\newcommand{\Tsft}{\T_{\!\mathit{sft}}}
\newcommand{\Tstck}{\T_{\mathit{l}}}
\newcommand{\TBstck}{{\boldsymbol\T}_{\!\mathit{l}}}

\newcommand{\seng}{\mathit{eng}}
\newcommand{\ssft}{\mathit{sft}}
\newcommand{\sgbx}{\mathit{gbx}}
\newcommand{\sveh}{\mathit{veh}}
\newcommand{\swhl}{\mathit{whl}}
\newcommand{\spri}{\mathit{pri}}
\newcommand{\ssec}{\mathit{sec}}
\newcommand{\skin}{\mathit{kin}}
\newcommand{\sstat}{\mathit{stat}}
\newcommand{\sstck}{\mathit{l}}
\newcommand{\sslip}{\mathit{s}}

\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Dataset}{\mathcal{D}}

\newcommand{\OPEN}{\textsc{Open}}
%\newcommand{\OPEN}{\mathrm{O\!P\!E\!N}}
\newcommand{\CLOSED}{\textsc{Closed}}	
%\newcommand{\CLOSED}{\textit{C\!L\!O\!S\!E\!D}}	

==> macros/tikzStyles.tex <==
\tikzstyle{s} = [font = \footnotesize]

\tikzstyle{doppelpfeil} = [-latex,postaction={draw,shorten >=6pt,-latex}]
\tikzstyle{sarrowtip} = [>=latex]  
\tikzstyle{myarrowtip} = [>=implies] 

\tikzset{curveinscope/.style={every path/.style={draw=white, double distance=1pt, line width=2pt, double=black, text=black}}}

\DeclareRobustCommand{\myLine}[1]{
(\tikzset{external/export next=false}\begin{tikzpicture}%
\useasboundingbox (-0.2ex,0) rectangle (4.65ex,1ex);%
\draw[line width=0.3ex,#1](0,0.65ex)--(4.5ex,0.65ex);%
\end{tikzpicture})}



